3D Multi-View Stylization with Pose-Free Correspondences Matching for Robust 3D Geometry Preservation

Artistic style transfer is well studied for images and videos, but extending it to multi-view 3D scenes remains difficult because stylization can disrupt correspondences needed by geometry-aware pipelines. Independent per-view stylization often causes texture drift, warped edges, and inconsistent shading, degrading SLAM, depth prediction, and multi-view reconstruction. This thesis addresses multi-view stylization that remains usable for downstream 3D tasks without assuming camera poses or an explicit 3D representation during training. We introduce a feed-forward stylization network trained with per-scene test-time optimization under a composite objective coupling appearance transfer with geometry preservation. Stylization is driven by an AdaIN-inspired loss from a frozen VGG-19 encoder, matching channel-wise moments to a style image. To stabilize structure across viewpoints, we propose a correspondence-based consistency loss using SuperPoint and SuperGlue, constraining descriptors from a stylized anchor view to remain consistent with matched descriptors from the original multi-view set. We also impose a depth-preservation loss using MiDaS/DPT and use global color alignment to reduce depth-model domain shift. A staged weight schedule introduces geometry and depth constraints. We evaluate on Tanks and Temples and Mip-NeRF 360 using image and reconstruction metrics. Style adherence and structure retention are measured by Color Histogram Distance (CHD) and Structure Distance (DSD). For 3D consistency, we use monocular DROID-SLAM trajectories and symmetric Chamfer distance on back-projected point clouds. Across ablations, correspondence and depth regularization reduce structural distortion and improve SLAM stability and reconstructed geometry; on scenes with MuVieCAST baselines, our method yields stronger trajectory and point-cloud consistency while maintaining competitive stylization.

==> chapters/01_introduction.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.

\chapter{Introduction}\label{chapter:introduction}
Use with pdfLaTeX and Biber.

\section{Section}
Citation test (with Biber)~\parencite{latex}.

\subsection{Subsection}

See~\autoref{tab:sample}, \autoref{fig:sample-drawing}, \autoref{fig:sample-plot}, \autoref{fig:sample-listing}, \autoref{fig:tum}, \autoref{fig:tumslide}.

\begin{table}[htpb]
  \caption[Example table]{An example for a simple table.}\label{tab:sample}
  \centering
  \begin{tabular}{l l l l}
    \toprule
      A & B & C & D \\
    \midrule
      1 & 2 & 1 & 2 \\
      2 & 3 & 2 & 3 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}[htpb]
  \centering
  % This should probably go into a file in figures/
  \begin{tikzpicture}[node distance=3cm]
    \node (R0) {$R_1$};
    \node (R1) [right of=R0] {$R_2$};
    \node (R2) [below of=R1] {$R_4$};
    \node (R3) [below of=R0] {$R_3$};
    \node (R4) [right of=R1] {$R_5$};

    \path[every node]
      (R0) edge (R1)
      (R0) edge (R3)
      (R3) edge (R2)
      (R2) edge (R1)
      (R1) edge (R4);
  \end{tikzpicture}
  \caption[Example drawing]{An example for a simple drawing.}\label{fig:sample-drawing}
\end{figure}

\begin{figure}[htpb]
  \centering

  \pgfplotstableset{col sep=&, row sep=\\}
  % This should probably go into a file in data/
  \pgfplotstableread{
    a & b    \\
    1 & 1000 \\
    2 & 1500 \\
    3 & 1600 \\
  }\exampleA
  \pgfplotstableread{
    a & b    \\
    1 & 1200 \\
    2 & 800 \\
    3 & 1400 \\
  }\exampleB
  % This should probably go into a file in figures/
  \begin{tikzpicture}
    \begin{axis}[
        ymin=0,
        legend style={legend pos=south east},
        grid,
        thick,
        ylabel=Y,
        xlabel=X
      ]
      \addplot table[x=a, y=b]{\exampleA};
      \addlegendentry{Example A};
      \addplot table[x=a, y=b]{\exampleB};
      \addlegendentry{Example B};
    \end{axis}
  \end{tikzpicture}
  \caption[Example plot]{An example for a simple plot.}\label{fig:sample-plot}
\end{figure}

\begin{figure}[htpb]
  \centering
  \begin{tabular}{c}
  \begin{lstlisting}[language=SQL]
    SELECT * FROM tbl WHERE tbl.str = "str"
  \end{lstlisting}
  \end{tabular}
  \caption[Example listing]{An example for a source code listing.}\label{fig:sample-listing}
\end{figure}

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{tum}
  \caption[Something else can be written here for listing this, otherwise the caption will be written!]{Includegraphics searches for the filename without extension first in logos, then in figures.} \label{fig:tum}
\end{figure}

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/tum}
  \caption{For pictures with the same name, the direct folder needs to be chosen.} \label{fig:tumslide}
\end{figure}

\begin{figure}[!tbp]
  \centering
  \subfloat[TUM Logo][The logo.]{\includegraphics[height=0.2\textheight]{tum}\label{fig:tum1}}
  \hfill
  \subfloat[TUM Slide][The famous slide.]{\includegraphics[height=0.2\textheight]{figures/tum}\label{fig:tum2}}
  \caption{Two TUM pictures side by side.}
  \label{fig:sidebyside}
\end{figure}

This is how the glossary will be used.

\Glspl{ddye}, \gls{r0}, \gls{R0}, and \gls{kdeac}. Also, the \glspl{tum} has many \glspl{computer}, not only one \Gls{computer}. Subsequent acronym usage will only print the short version of \glspl{tuma} (take care of plural, if needed!), like here with \gls{tuma}, too. It can also be --> \glsdisp{tum}{hidden}\footnote{Example for a hidden TUM glossary entry.} <--.

\todo{Now it is your turn to write your thesis.

This will be a few tough weeks.}

\done{Nevertheless, celebrate it when it is done!}


==> chapters/background.tex <==
\chapter{Background}
\section{Neural Style Transfer}
A common formulation represents content and style using feature activations of a fixed classification network (e.g., VGG). For a content image $I$ and style image $S$, a stylized output $\hat{I}$ is obtained by minimizing:
\begin{equation}
\mathcal{L}(\hat{I}) = \lambda_c \mathcal{L}_{content}(\hat{I}, I) + \lambda_s \mathcal{L}_{style}(\hat{I}, S).
\end{equation}
Content losses typically match deep feature activations; style losses match statistics (e.g., Gram matrices) of features across layers.

\section{Adaptive Instance Normalization (AdaIN)}
AdaIN performs a channel-wise affine transform in feature space to match the mean and variance of content features to those of style features. Denote content features $f_c \in \mathbb{R}^{C\times HW}$ and style features $f_s$. Let $\mu(\cdot)$ and $\sigma(\cdot)$ be per-channel mean and standard deviation. AdaIN is:
\begin{equation}
\text{AdaIN}(f_c, f_s) = \sigma(f_s)\left(\frac{f_c - \mu(f_c)}{\sigma(f_c) + \epsilon}\right) + \mu(f_s).
\end{equation}
This thesis uses an AdaIN-like \emph{loss} that matches feature statistics rather than explicitly inserting AdaIN layers into the network.

\section{Multi-View Correspondences}
Given two images of the same scene with overlap, local feature detectors/descriptors and matchers provide correspondences $\{(x^A_k, x^B_k)\}$. High-quality correspondences are central to enforcing view consistency: the stylized appearance near $x^A_k$ should remain compatible with that near $x^B_k$.

\section{Monocular Depth Priors}
Modern monocular depth networks (e.g., MiDaS/DPT) output dense depth/disparity predictions from a single image. Although scale may be ambiguous, relative depth structure provides a useful prior to discourage stylization from introducing non-physical deformations.

\section{SLAM-Based Consistency Evaluation}
To test whether stylization preserves geometry, we can run the same SLAM pipeline on original and stylized sequences and measure how closely their reconstructions agree after alignment. This thesis uses trajectory alignment metrics and point-cloud distances.


==> chapters/intro.tex <==
\chapter{Introduction}
\section{Motivation}

The research domain of Computer Vision that involves in migrating the intriguing textures of a style image to a reference image, while
preserving its original geometrical semantics is image style transfer. Neural style transfer involves deployment of deep convolutional neural networks (CNN) for stylizing. The performance of these methods is impressive in stylizing 2D images with diverse style textures[cite]. When deployed on videos or multi-view captures of a 3D scene, per-frame/per-view stylization commonly yields temporal flicker and view-dependent artifacts: edges bend, textures ``swim'' across surfaces, and fine structures appear or disappear depending on viewpoint. Now to migrate from the 2D scenes to 3D scenes, various authors have proposed 3D stylization methods [cite], which operate on various inputs like point cloud[PSNet: A Style Transfer Network for Point Cloud Stylization
on Geometry and Color, Learning to Stylize Novel Views,  Point-based neural rendering with perview optimization ], meshes [Style transfer for indoor 3d scene reconstructions. ], neural radiance fields [ Stylizednerf: Consistent 3d scene stylization as stylized nerf via 2d-3d mutual learning., Arf: Artistic radiance
fields.], gaussian splatting[stylizedgs2024, G-style, stylegaussian2024], and multi-view images [muviecast, osdiffst]. 

The key challenges faced generally in most 2D stylization objectives do not enforce that surface points retain stable appearance across views. A texture pattern that looks plausible in one view may shift in another. Style transfer can modify edges and high-frequency cues used
by keypoint detectors and matchers, reducing correspondence quality and harming camera
tracking. Stylization can alter shading and contrast in ways that confuse monocular
depth priors, causing inconsistent depth estimates that affect 3D fusion. 

The recent methods of a scene stylization involve Nerfs and Gaussian Splatting that ..... These methods show reliable performance in scene stylization but these methods lack conviction. The gaussian splatting methods require the camera positions as well as the Sfms for creation of the whole scene. Another drawback is that this method involves in blurring out the stylized images where there is a loss in the edges and high-frequency components. Also considering the video stylization methods, these introduce temporal stabilization techniques but they require a smooth transition in frames so that the stabilization is valid. But all of these methods has some or the other constraints of requiring additional information other than the multi-view images. The recent research direction of multi-view stylization involves methods [cite muvie, osdf], that incorporate camera poses for stylization and geometry preservation. The authors of [ostdiff], has introduced a diffusion based framework for multi-view stylization but the diffusion based methods are often prone to generating artifacts that breaks the integrity of an object and is less suitable for 3d realted downstream tasks after stylization. 

Also, in literature the standard method of evaluating the stylization efficacy is the FID (frechet Inception score), this measures how much the stylized image is closer to the original rgb image in terms of its content semantics. Also for multi-view stylization research, the recent method [muvie], adapted to use humans to measure how good the stylization is. Based on the human score they prersented their results. The paper [osdiff], has resorted to use CHD (color histogram distance) for measurement of the stylization and DSD (Dino structure distance) for measuring how much the structure of a stylized image is close to its rgb counter part. But these are all single image based evaluations and does not give a clear picture regarding the 3d world's integrity after stylization. To reconstruct the 3d world from these stylized images, we need a measurement of how good the method in terms of stylization as well as in preserving the geometry for 3d integrity.  

So in this regard we propose a novel multi-view images based stylization methodology that is independent of the camera poses and any other information, while preserving the geometric integrity of the 3d scene. We have proposed a novel superpoint/superglue based geometric loss that penalizes the stylizer network to preserve the geometric constraints in the stylized image via feature based correspondences matching. 

Also in most of the multi-view stylization models, the stylizer network is trained only on a single style and single scene and this would increase the number of runs/memory usage over prolonged time. So, in this regard we change our stylizer network to a conditional unet where we have multiple styles and train a single scene over these styles and we show that our method is capable of transferring our stylization to unknown scenes during testing while preserving geometry to a good extent. 

To measure the structural geometric information of the 3d world from the -- slams are mostly based on feature matching and point correspondences -- so a comparison of slam trajectory of the original rgb images and the stylized images would measure how much structural integrity is preserved in the stylized images for 3d based reconstruction or how close it is to the geometry of the 3d world. We leverage monocular DROID-SLAM as our assumptions were with pose-free scenes understanding. Leveraging the DROID-SLAM, we also recompute the point clouds from the rgb images and the stylized images, a closer structural similarity would indicate a much better 3d reconstruction and geometry preservation. 

% style transfer 2d-3d
% types of 3d style transfer
% multiview setup
% problems with existing methods
% then evaluation metrics not suff

% Artistic style transfer aims to synthesize an image that preserves the semantic content of a photograph while adopting the appearance characteristics of an artwork. While early neural style transfer methods produced impressive results, they were typically designed for single images. 

% These inconsistencies are not only visually distracting; they also break the assumptions of geometry-aware pipelines such as SLAM, multi-view stereo, and neural rendering. -- good

Multi-view consistent stylization is particularly relevant in modern 3D vision and graphics. Large-scale reconstructions are increasingly built from casually captured videos, and downstream applications often require novel-view synthesis, mesh extraction, or point cloud fusion. If stylization destroys cross-view correspondences or alters depth cues, reconstruction quality can degrade drastically. This thesis targets the following question:

\begin{quote}
\textit{How can we obtain multi-view artistic stylization that is visually stylized yet preserves geometric consistency sufficiently for downstream 3D reconstruction? How to measure in what extent the geometry is preserved while stylizing?}
\end{quote}

\section{Problem Statement}
Given a set of RGB images $\{I_i\}_{i=1}^N$ of the same static scene captured from different viewpoints and a single style reference image $S$, our goal is to produce stylized views $\{\hat{I}_i\}_{i=1}^N$ such that:
\begin{enumerate}
    \item Each $\hat{I}_i$ reflects the style of $S$,
    \item $\hat{I}_i$ preserves the scene structure of $I_i$,
    \item The collection $\{\hat{I}_i\}$ is consistent across views, i.e., corresponding 3D points have compatible appearance under viewpoint changes.
\end{enumerate}

So as to summarize our thesis contributions:
\section{Thesis Contributions}
This thesis makes the following contributions:
\begin{enumerate}
    \item \textbf{A lightweight per-scene stylization network} trained with an AdaIN-inspired feature-statistics objective for fast stylization.
    \item \textbf{A correspondence-based multi-view consistency loss} using SuperPoint/SuperGlue matches to explicitly regularize feature stability across views.
    \item \textbf{A depth-preservation loss} using a frozen MiDaS/DPT model to penalize stylization-induced depth distortions.
    \item \textbf{A practical domain-alignment step} (dataset-to-style color transfer) to reduce depth-model domain shift during training.
    \item \textbf{A quantitative evaluation protocol} spanning static style/structure metrics (CHD, DSD) and dynamic 3D consistency metrics (ATE/RTE and Chamfer distance) from DROID-SLAM reconstructions.
\end{enumerate}

\section{Why This Direction Matters}
Unlike methods that only optimize perceptual stylization, the proposed approach is explicitly designed for \emph{downstream geometric usability}. In applications such as stylized 3D reconstruction, AR/VR content creation, and artistic scene capture, it is not enough for each image to look stylized independently---the stylization must be coherent across viewpoints.

\section{Thesis Outline}
Chapter~2 reviews background on neural style transfer and multi-view geometry. Chapter~3 surveys related work, including multi-view consistent stylization and diffusion-based methods. Chapter~4 details the proposed method. Chapters~5--7 describe experimental setup, evaluation metrics, and quantitative results. Chapter~8 discusses limitations and future work. Qualitative analysis is left as a placeholder to be completed once figures are finalized.

